On the nature of the stock market: Simulations and experiments

In this dissertation two simple models of stock exchange are developed and simulated numerically. The first is characterized by centralized trading with a market maker. Unfortunately, this model is unable to generate realistic market dynamics. The second model discards the requirement of centralized trading. Under variation of the control parameter the model exhibits two phase transitions: both a first- and a second-order (critical). The decentralized model is able to capture many of the interesting properties observed in empirical markets. Significantly, these properties only emerge when the parameters are tuned such that the model spans the critical point. This suggests that real markets may operate at or near a critical point, but is unable to explain why this should be. One of the main points of the thesis is that these empirical phenomena are not present in the stochastic driving force, but emerge endogenously from interactions between agents.

==> chResults/csemMaxTransS.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup%
  \makeatletter%
  \newcommand{\GNUPLOTspecial}{%
    \@sanitize\catcode`\%=14\relax\special}%
  \setlength{\unitlength}{0.1bp}%
{\GNUPLOTspecial{!
%!PS-Adobe-2.0 EPSF-2.0
%%Title: csemMaxTransS.tex
%%Creator: gnuplot 3.7 patchlevel 1
%%CreationDate: Sun May 28 01:06:12 2000
%%DocumentFonts: 
%%BoundingBox: 0 0 360 216
%%Orientation: Landscape
%%EndComments
/gnudict 256 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/vshift -33 def
/dl {10 mul} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/UP { dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke userlinewidth 2 mul setlinewidth } def
/AL { stroke userlinewidth 2 div setlinewidth } def
/UL { dup gnulinewidth mul /userlinewidth exch def
      10 mul /udl exch def } def
/PL { stroke userlinewidth setlinewidth } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 udl mul 2 udl mul] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 1 0 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 1 0 DL } def
/LT2 { PL [2 dl 3 dl] 0 0 1 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/Pnt { stroke [] 0 setdash
   gsave 1 setlinecap M 0 0 V stroke grestore } def
/Dia { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt } def
/Pls { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/Box { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt } def
/Crs { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/TriU { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt  } def
/Star { 2 copy Pls Crs } def
/BoxF { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V  hpt2 0 V  0 vpt2 V
  hpt2 neg 0 V  closepath fill } def
/TriUF { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill } def
/TriD { stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt  } def
/TriDF { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill } def
/Pent { stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt } def
/PentF { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore } def
/Circle { stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt } def
/CircleF { stroke [] 0 setdash hpt 0 360 arc fill } def
/C0 { BL [] 0 setdash 2 copy moveto vpt 90 450  arc } bind def
/C1 { BL [] 0 setdash 2 copy        moveto
       2 copy  vpt 0 90 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C2 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C3 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C4 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C5 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 90 arc
       2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc } bind def
/C6 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 90 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C7 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 0 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C8 { BL [] 0 setdash 2 copy moveto
      2 copy vpt 270 360 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C9 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 270 450 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C10 { BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
       2 copy moveto
       2 copy vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C11 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
       2 copy moveto
       2 copy  vpt 270 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C12 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C13 { BL [] 0 setdash  2 copy moveto
       2 copy  vpt 0 90 arc closepath fill
       2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C14 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 360 arc closepath fill
               vpt 0 360 arc } bind def
/C15 { BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/Rec   { newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
       neg 0 rlineto closepath } bind def
/Square { dup Rec } bind def
/Bsquare { vpt sub exch vpt sub exch vpt2 Square } bind def
/S0 { BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare } bind def
/S1 { BL [] 0 setdash 2 copy vpt Square fill Bsquare } bind def
/S2 { BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S3 { BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare } bind def
/S4 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S5 { BL [] 0 setdash 2 copy 2 copy vpt Square fill
       exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S6 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S7 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
       2 copy vpt Square fill
       Bsquare } bind def
/S8 { BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare } bind def
/S9 { BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S10 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
       Bsquare } bind def
/S11 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
       Bsquare } bind def
/S12 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare } bind def
/S13 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy vpt Square fill Bsquare } bind def
/S14 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S15 { BL [] 0 setdash 2 copy Bsquare fill Bsquare } bind def
/D0 { gsave translate 45 rotate 0 0 S0 stroke grestore } bind def
/D1 { gsave translate 45 rotate 0 0 S1 stroke grestore } bind def
/D2 { gsave translate 45 rotate 0 0 S2 stroke grestore } bind def
/D3 { gsave translate 45 rotate 0 0 S3 stroke grestore } bind def
/D4 { gsave translate 45 rotate 0 0 S4 stroke grestore } bind def
/D5 { gsave translate 45 rotate 0 0 S5 stroke grestore } bind def
/D6 { gsave translate 45 rotate 0 0 S6 stroke grestore } bind def
/D7 { gsave translate 45 rotate 0 0 S7 stroke grestore } bind def
/D8 { gsave translate 45 rotate 0 0 S8 stroke grestore } bind def
/D9 { gsave translate 45 rotate 0 0 S9 stroke grestore } bind def
/D10 { gsave translate 45 rotate 0 0 S10 stroke grestore } bind def
/D11 { gsave translate 45 rotate 0 0 S11 stroke grestore } bind def
/D12 { gsave translate 45 rotate 0 0 S12 stroke grestore } bind def
/D13 { gsave translate 45 rotate 0 0 S13 stroke grestore } bind def
/D14 { gsave translate 45 rotate 0 0 S14 stroke grestore } bind def
/D15 { gsave translate 45 rotate 0 0 S15 stroke grestore } bind def
/DiaE { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke } def
/BoxE { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke } def
/TriUE { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke } def
/TriDE { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke } def
/PentE { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore } def
/CircE { stroke [] 0 setdash 
  hpt 0 360 arc stroke } def
/Opaque { gsave closepath 1 setgray fill grestore 0 setgray closepath } def
/DiaW { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke } def
/BoxW { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke } def
/TriUW { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke } def
/TriDW { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke } def
/PentW { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore } def
/CircW { stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke } def
/BoxFill { gsave Rec 1 setgray fill grestore } def
end
%%EndProlog
}}%
\begin{picture}(3600,2160)(0,0)%
{\GNUPLOTspecial{"
gnudict begin
gsave
0 0 translate
0.100 0.100 scale
0 setgray
newpath
1.000 UL
LTb
750 521 M
63 0 V
2637 0 R
-63 0 V
750 1291 M
63 0 V
2637 0 R
-63 0 V
750 2060 M
63 0 V
2637 0 R
-63 0 V
750 300 M
0 63 V
0 1697 R
0 -63 V
1290 300 M
0 63 V
0 1697 R
0 -63 V
1830 300 M
0 63 V
0 1697 R
0 -63 V
2370 300 M
0 63 V
0 1697 R
0 -63 V
2910 300 M
0 63 V
0 1697 R
0 -63 V
3450 300 M
0 63 V
0 1697 R
0 -63 V
1.000 UL
LTb
750 300 M
2700 0 V
0 1760 V
-2700 0 V
750 300 L
1.000 UP
1.000 UL
LT0
1098 1378 Pls
1638 1542 Pls
2178 1007 Pls
2892 795 Pls
3432 561 Pls
3218 1947 Pls
1.000 UL
LT1
3087 1847 M
263 0 V
1098 1520 M
23 -10 V
24 -9 V
23 -10 V
24 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
24 -9 V
23 -10 V
24 -9 V
23 -10 V
24 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
23 -9 V
24 -10 V
24 -9 V
stroke
grestore
end
showpage
}}%
\put(3037,1847){\makebox(0,0)[r]{Power law exponent = $-0.14\pm 0.06$}}%
\put(3037,1947){\makebox(0,0)[r]{Data}}%
\put(2100,50){\makebox(0,0){Number of agents $N$}}%
\put(100,1180){%
\special{ps: gsave currentpoint currentpoint translate
270 rotate neg exch neg exch translate}%
\makebox(0,0)[b]{\shortstack{Saturated forecast error $\sigma_{\epsilon,min}$}}%
\special{ps: currentpoint grestore moveto}%
}%
\put(3450,200){\makebox(0,0){1024}}%
\put(2910,200){\makebox(0,0){512}}%
\put(2370,200){\makebox(0,0){256}}%
\put(1830,200){\makebox(0,0){128}}%
\put(1290,200){\makebox(0,0){64}}%
\put(750,200){\makebox(0,0){32}}%
\put(700,2060){\makebox(0,0)[r]{$2^{-5/2}$}}%
\put(700,1291){\makebox(0,0)[r]{$2^{-6/2}$}}%
\put(700,521){\makebox(0,0)[r]{$2^{-7/2}$}}%
\end{picture}%
\endgroup
\endinput


==> chResults/csemSteadyPrice.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup%
  \makeatletter%
  \newcommand{\GNUPLOTspecial}{%
    \@sanitize\catcode`\%=14\relax\special}%
  \setlength{\unitlength}{0.1bp}%
{\GNUPLOTspecial{!
%!PS-Adobe-2.0 EPSF-2.0
%%Title: csemSteadyPrice.tex
%%Creator: gnuplot 3.7 patchlevel 1
%%CreationDate: Sat May 27 12:14:39 2000
%%DocumentFonts: 
%%BoundingBox: 0 0 360 216
%%Orientation: Landscape
%%EndComments
/gnudict 256 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/vshift -33 def
/dl {10 mul} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/UP { dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke userlinewidth 2 mul setlinewidth } def
/AL { stroke userlinewidth 2 div setlinewidth } def
/UL { dup gnulinewidth mul /userlinewidth exch def
      10 mul /udl exch def } def
/PL { stroke userlinewidth setlinewidth } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 udl mul 2 udl mul] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 1 0 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 1 0 DL } def
/LT2 { PL [2 dl 3 dl] 0 0 1 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/Pnt { stroke [] 0 setdash
   gsave 1 setlinecap M 0 0 V stroke grestore } def
/Dia { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt } def
/Pls { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/Box { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt } def
/Crs { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/TriU { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt  } def
/Star { 2 copy Pls Crs } def
/BoxF { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V  hpt2 0 V  0 vpt2 V
  hpt2 neg 0 V  closepath fill } def
/TriUF { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill } def
/TriD { stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt  } def
/TriDF { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill } def
/Pent { stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt } def
/PentF { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore } def
/Circle { stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt } def
/CircleF { stroke [] 0 setdash hpt 0 360 arc fill } def
/C0 { BL [] 0 setdash 2 copy moveto vpt 90 450  arc } bind def
/C1 { BL [] 0 setdash 2 copy        moveto
       2 copy  vpt 0 90 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C2 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C3 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C4 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C5 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 90 arc
       2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc } bind def
/C6 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 90 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C7 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 0 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C8 { BL [] 0 setdash 2 copy moveto
      2 copy vpt 270 360 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C9 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 270 450 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C10 { BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
       2 copy moveto
       2 copy vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C11 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
       2 copy moveto
       2 copy  vpt 270 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C12 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C13 { BL [] 0 setdash  2 copy moveto
       2 copy  vpt 0 90 arc closepath fill
       2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C14 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 360 arc closepath fill
               vpt 0 360 arc } bind def
/C15 { BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/Rec   { newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
       neg 0 rlineto closepath } bind def
/Square { dup Rec } bind def
/Bsquare { vpt sub exch vpt sub exch vpt2 Square } bind def
/S0 { BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare } bind def
/S1 { BL [] 0 setdash 2 copy vpt Square fill Bsquare } bind def
/S2 { BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S3 { BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare } bind def
/S4 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S5 { BL [] 0 setdash 2 copy 2 copy vpt Square fill
       exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S6 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S7 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
       2 copy vpt Square fill
       Bsquare } bind def
/S8 { BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare } bind def
/S9 { BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S10 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
       Bsquare } bind def
/S11 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
       Bsquare } bind def
/S12 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare } bind def
/S13 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy vpt Square fill Bsquare } bind def
/S14 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S15 { BL [] 0 setdash 2 copy Bsquare fill Bsquare } bind def
/D0 { gsave translate 45 rotate 0 0 S0 stroke grestore } bind def
/D1 { gsave translate 45 rotate 0 0 S1 stroke grestore } bind def
/D2 { gsave translate 45 rotate 0 0 S2 stroke grestore } bind def
/D3 { gsave translate 45 rotate 0 0 S3 stroke grestore } bind def
/D4 { gsave translate 45 rotate 0 0 S4 stroke grestore } bind def
/D5 { gsave translate 45 rotate 0 0 S5 stroke grestore } bind def
/D6 { gsave translate 45 rotate 0 0 S6 stroke grestore } bind def
/D7 { gsave translate 45 rotate 0 0 S7 stroke grestore } bind def
/D8 { gsave translate 45 rotate 0 0 S8 stroke grestore } bind def
/D9 { gsave translate 45 rotate 0 0 S9 stroke grestore } bind def
/D10 { gsave translate 45 rotate 0 0 S10 stroke grestore } bind def
/D11 { gsave translate 45 rotate 0 0 S11 stroke grestore } bind def
/D12 { gsave translate 45 rotate 0 0 S12 stroke grestore } bind def
/D13 { gsave translate 45 rotate 0 0 S13 stroke grestore } bind def
/D14 { gsave translate 45 rotate 0 0 S14 stroke grestore } bind def
/D15 { gsave translate 45 rotate 0 0 S15 stroke grestore } bind def
/DiaE { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke } def
/BoxE { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke } def
/TriUE { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke } def
/TriDE { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke } def
/PentE { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore } def
/CircE { stroke [] 0 setdash 
  hpt 0 360 arc stroke } def
/Opaque { gsave closepath 1 setgray fill grestore 0 setgray closepath } def
/DiaW { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke } def
/BoxW { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke } def
/TriUW { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke } def
/TriDW { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke } def
/PentW { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore } def
/CircW { stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke } def
/BoxFill { gsave Rec 1 setgray fill grestore } def
end
%%EndProlog
}}%
\begin{picture}(3600,2160)(0,0)%
{\GNUPLOTspecial{"
gnudict begin
gsave
0 0 translate
0.100 0.100 scale
0 setgray
newpath
1.000 UL
LTb
400 300 M
63 0 V
2987 0 R
-63 0 V
400 477 M
31 0 V
3019 0 R
-31 0 V
400 580 M
31 0 V
3019 0 R
-31 0 V
400 653 M
31 0 V
3019 0 R
-31 0 V
400 710 M
31 0 V
3019 0 R
-31 0 V
400 757 M
31 0 V
3019 0 R
-31 0 V
400 796 M
31 0 V
3019 0 R
-31 0 V
400 830 M
31 0 V
3019 0 R
-31 0 V
400 860 M
31 0 V
3019 0 R
-31 0 V
400 887 M
63 0 V
2987 0 R
-63 0 V
400 1063 M
31 0 V
3019 0 R
-31 0 V
400 1167 M
31 0 V
3019 0 R
-31 0 V
400 1240 M
31 0 V
3019 0 R
-31 0 V
400 1297 M
31 0 V
3019 0 R
-31 0 V
400 1343 M
31 0 V
3019 0 R
-31 0 V
400 1382 M
31 0 V
3019 0 R
-31 0 V
400 1416 M
31 0 V
3019 0 R
-31 0 V
400 1446 M
31 0 V
3019 0 R
-31 0 V
400 1473 M
63 0 V
2987 0 R
-63 0 V
400 1650 M
31 0 V
3019 0 R
-31 0 V
400 1753 M
31 0 V
3019 0 R
-31 0 V
400 1827 M
31 0 V
3019 0 R
-31 0 V
400 1883 M
31 0 V
3019 0 R
-31 0 V
400 1930 M
31 0 V
3019 0 R
-31 0 V
400 1969 M
31 0 V
3019 0 R
-31 0 V
400 2003 M
31 0 V
3019 0 R
-31 0 V
400 2033 M
31 0 V
3019 0 R
-31 0 V
400 2060 M
63 0 V
2987 0 R
-63 0 V
400 300 M
0 63 V
0 1697 R
0 -63 V
1417 300 M
0 63 V
0 1697 R
0 -63 V
2433 300 M
0 63 V
0 1697 R
0 -63 V
3450 300 M
0 63 V
0 1697 R
0 -63 V
1.000 UL
LTb
400 300 M
3050 0 V
0 1760 V
-3050 0 V
400 300 L
1.000 UP
1.000 UL
LT0
566 1530 Pls
762 1587 Pls
935 1392 Pls
1089 1392 Pls
1229 1446 Pls
1357 1282 Pls
1474 1310 Pls
1583 1231 Pls
1684 1097 Pls
1779 1074 Pls
1868 1041 Pls
1952 972 Pls
2031 978 Pls
2106 894 Pls
2178 889 Pls
2246 819 Pls
2311 814 Pls
2373 792 Pls
2433 747 Pls
2491 753 Pls
2546 712 Pls
2600 702 Pls
2651 671 Pls
2701 672 Pls
2749 657 Pls
2795 663 Pls
2841 640 Pls
2884 633 Pls
2927 605 Pls
2968 610 Pls
3008 600 Pls
3047 587 Pls
3086 566 Pls
3123 569 Pls
3159 545 Pls
3194 561 Pls
3229 554 Pls
3263 539 Pls
3295 540 Pls
3328 524 Pls
3359 520 Pls
3390 527 Pls
3420 502 Pls
3450 491 Pls
3218 1947 Pls
1.000 UP
1.000 UL
LT1
762 1617 Crs
935 1518 Crs
1089 1334 Crs
1229 1322 Crs
1357 1286 Crs
1474 1176 Crs
1583 1150 Crs
1684 1070 Crs
1779 1014 Crs
1868 976 Crs
1952 911 Crs
2031 879 Crs
2106 866 Crs
2178 817 Crs
2246 785 Crs
2311 780 Crs
2373 729 Crs
2433 735 Crs
3218 1847 Crs
1.000 UP
1.000 UL
LT2
566 1711 Star
762 1577 Star
935 1455 Star
1089 1347 Star
1229 1239 Star
1357 1148 Star
1474 1045 Star
1583 1008 Star
1684 963 Star
1779 922 Star
1868 885 Star
1952 845 Star
2031 826 Star
2106 799 Star
2178 776 Star
2246 749 Star
2311 730 Star
2373 719 Star
2433 696 Star
3218 1747 Star
1.000 UP
1.000 UL
LT3
566 1709 Box
762 1504 Box
935 1367 Box
1089 1187 Box
1229 1039 Box
1357 980 Box
1474 944 Box
1583 913 Box
1684 887 Box
1779 869 Box
1868 842 Box
1952 823 Box
2031 796 Box
2106 778 Box
2178 757 Box
2246 742 Box
2311 722 Box
2373 709 Box
2433 698 Box
3218 1647 Box
stroke
grestore
end
showpage
}}%
\put(3037,1647){\makebox(0,0)[r]{$N=1000$}}%
\put(3037,1747){\makebox(0,0)[r]{$N=500$}}%
\put(3037,1847){\makebox(0,0)[r]{$N=200$}}%
\put(3037,1947){\makebox(0,0)[r]{$N=100$}}%
\put(1925,50){\makebox(0,0){Forecast error $\sigma_\epsilon$}}%
\put(100,1180){%
\special{ps: gsave currentpoint currentpoint translate
270 rotate neg exch neg exch translate}%
\makebox(0,0)[b]{\shortstack{Steady-state price}}%
\special{ps: currentpoint grestore moveto}%
}%
\put(3450,200){\makebox(0,0){$2^{-1}$}}%
\put(2433,200){\makebox(0,0){$2^{-2}$}}%
\put(1417,200){\makebox(0,0){$2^{-3}$}}%
\put(400,200){\makebox(0,0){$2^{-4}$}}%
\put(350,2060){\makebox(0,0)[r]{100}}%
\put(350,1473){\makebox(0,0)[r]{10}}%
\put(350,887){\makebox(0,0)[r]{1}}%
\put(350,300){\makebox(0,0)[r]{0.1}}%
\end{picture}%
\endgroup
\endinput


==> chResults2/csemCrashes0.10.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup%
  \makeatletter%
  \newcommand{\GNUPLOTspecial}{%
    \@sanitize\catcode`\%=14\relax\special}%
  \setlength{\unitlength}{0.1bp}%
{\GNUPLOTspecial{!
%!PS-Adobe-2.0 EPSF-2.0
%%Title: csemCrashes0.10.tex
%%Creator: gnuplot 3.7 patchlevel 1
%%CreationDate: Fri Jun 09 22:08:24 2000
%%DocumentFonts: 
%%BoundingBox: 0 0 360 216
%%Orientation: Landscape
%%EndComments
/gnudict 256 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/vshift -33 def
/dl {10 mul} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/UP { dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke userlinewidth 2 mul setlinewidth } def
/AL { stroke userlinewidth 2 div setlinewidth } def
/UL { dup gnulinewidth mul /userlinewidth exch def
      10 mul /udl exch def } def
/PL { stroke userlinewidth setlinewidth } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 udl mul 2 udl mul] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 1 0 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 1 0 DL } def
/LT2 { PL [2 dl 3 dl] 0 0 1 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/Pnt { stroke [] 0 setdash
   gsave 1 setlinecap M 0 0 V stroke grestore } def
/Dia { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt } def
/Pls { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/Box { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt } def
/Crs { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/TriU { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt  } def
/Star { 2 copy Pls Crs } def
/BoxF { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V  hpt2 0 V  0 vpt2 V
  hpt2 neg 0 V  closepath fill } def
/TriUF { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill } def
/TriD { stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt  } def
/TriDF { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill } def
/Pent { stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt } def
/PentF { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore } def
/Circle { stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt } def
/CircleF { stroke [] 0 setdash hpt 0 360 arc fill } def
/C0 { BL [] 0 setdash 2 copy moveto vpt 90 450  arc } bind def
/C1 { BL [] 0 setdash 2 copy        moveto
       2 copy  vpt 0 90 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C2 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C3 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C4 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C5 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 90 arc
       2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc } bind def
/C6 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 90 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C7 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 0 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C8 { BL [] 0 setdash 2 copy moveto
      2 copy vpt 270 360 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C9 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 270 450 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C10 { BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
       2 copy moveto
       2 copy vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C11 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
       2 copy moveto
       2 copy  vpt 270 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C12 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C13 { BL [] 0 setdash  2 copy moveto
       2 copy  vpt 0 90 arc closepath fill
       2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C14 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 360 arc closepath fill
               vpt 0 360 arc } bind def
/C15 { BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/Rec   { newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
       neg 0 rlineto closepath } bind def
/Square { dup Rec } bind def
/Bsquare { vpt sub exch vpt sub exch vpt2 Square } bind def
/S0 { BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare } bind def
/S1 { BL [] 0 setdash 2 copy vpt Square fill Bsquare } bind def
/S2 { BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S3 { BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare } bind def
/S4 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S5 { BL [] 0 setdash 2 copy 2 copy vpt Square fill
       exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S6 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S7 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
       2 copy vpt Square fill
       Bsquare } bind def
/S8 { BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare } bind def
/S9 { BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S10 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
       Bsquare } bind def
/S11 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
       Bsquare } bind def
/S12 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare } bind def
/S13 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy vpt Square fill Bsquare } bind def
/S14 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S15 { BL [] 0 setdash 2 copy Bsquare fill Bsquare } bind def
/D0 { gsave translate 45 rotate 0 0 S0 stroke grestore } bind def
/D1 { gsave translate 45 rotate 0 0 S1 stroke grestore } bind def
/D2 { gsave translate 45 rotate 0 0 S2 stroke grestore } bind def
/D3 { gsave translate 45 rotate 0 0 S3 stroke grestore } bind def
/D4 { gsave translate 45 rotate 0 0 S4 stroke grestore } bind def
/D5 { gsave translate 45 rotate 0 0 S5 stroke grestore } bind def
/D6 { gsave translate 45 rotate 0 0 S6 stroke grestore } bind def
/D7 { gsave translate 45 rotate 0 0 S7 stroke grestore } bind def
/D8 { gsave translate 45 rotate 0 0 S8 stroke grestore } bind def
/D9 { gsave translate 45 rotate 0 0 S9 stroke grestore } bind def
/D10 { gsave translate 45 rotate 0 0 S10 stroke grestore } bind def
/D11 { gsave translate 45 rotate 0 0 S11 stroke grestore } bind def
/D12 { gsave translate 45 rotate 0 0 S12 stroke grestore } bind def
/D13 { gsave translate 45 rotate 0 0 S13 stroke grestore } bind def
/D14 { gsave translate 45 rotate 0 0 S14 stroke grestore } bind def
/D15 { gsave translate 45 rotate 0 0 S15 stroke grestore } bind def
/DiaE { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke } def
/BoxE { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke } def
/TriUE { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke } def
/TriDE { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke } def
/PentE { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore } def
/CircE { stroke [] 0 setdash 
  hpt 0 360 arc stroke } def
/Opaque { gsave closepath 1 setgray fill grestore 0 setgray closepath } def
/DiaW { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke } def
/BoxW { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke } def
/TriUW { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke } def
/TriDW { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke } def
/PentW { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore } def
/CircW { stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke } def
/BoxFill { gsave Rec 1 setgray fill grestore } def
end
%%EndProlog
}}%
\begin{picture}(3600,2160)(0,0)%
{\GNUPLOTspecial{"
gnudict begin
gsave
0 0 translate
0.100 0.100 scale
0 setgray
newpath
1.000 UL
LTb
450 300 M
63 0 V
2937 0 R
-63 0 V
450 432 M
31 0 V
2969 0 R
-31 0 V
450 510 M
31 0 V
2969 0 R
-31 0 V
450 565 M
31 0 V
2969 0 R
-31 0 V
450 608 M
31 0 V
2969 0 R
-31 0 V
450 642 M
31 0 V
2969 0 R
-31 0 V
450 672 M
31 0 V
2969 0 R
-31 0 V
450 697 M
31 0 V
2969 0 R
-31 0 V
450 720 M
31 0 V
2969 0 R
-31 0 V
450 740 M
63 0 V
2937 0 R
-63 0 V
450 872 M
31 0 V
2969 0 R
-31 0 V
450 950 M
31 0 V
2969 0 R
-31 0 V
450 1005 M
31 0 V
2969 0 R
-31 0 V
450 1048 M
31 0 V
2969 0 R
-31 0 V
450 1082 M
31 0 V
2969 0 R
-31 0 V
450 1112 M
31 0 V
2969 0 R
-31 0 V
450 1137 M
31 0 V
2969 0 R
-31 0 V
450 1160 M
31 0 V
2969 0 R
-31 0 V
450 1180 M
63 0 V
2937 0 R
-63 0 V
450 1312 M
31 0 V
2969 0 R
-31 0 V
450 1390 M
31 0 V
2969 0 R
-31 0 V
450 1445 M
31 0 V
2969 0 R
-31 0 V
450 1488 M
31 0 V
2969 0 R
-31 0 V
450 1522 M
31 0 V
2969 0 R
-31 0 V
450 1552 M
31 0 V
2969 0 R
-31 0 V
450 1577 M
31 0 V
2969 0 R
-31 0 V
450 1600 M
31 0 V
2969 0 R
-31 0 V
450 1620 M
63 0 V
2937 0 R
-63 0 V
450 1752 M
31 0 V
2969 0 R
-31 0 V
450 1830 M
31 0 V
2969 0 R
-31 0 V
450 1885 M
31 0 V
2969 0 R
-31 0 V
450 1928 M
31 0 V
2969 0 R
-31 0 V
450 1962 M
31 0 V
2969 0 R
-31 0 V
450 1992 M
31 0 V
2969 0 R
-31 0 V
450 2017 M
31 0 V
2969 0 R
-31 0 V
450 2040 M
31 0 V
2969 0 R
-31 0 V
450 2060 M
63 0 V
2937 0 R
-63 0 V
450 300 M
0 63 V
0 1697 R
0 -63 V
750 300 M
0 63 V
0 1697 R
0 -63 V
1050 300 M
0 63 V
0 1697 R
0 -63 V
1350 300 M
0 63 V
0 1697 R
0 -63 V
1650 300 M
0 63 V
0 1697 R
0 -63 V
1950 300 M
0 63 V
0 1697 R
0 -63 V
2250 300 M
0 63 V
0 1697 R
0 -63 V
2550 300 M
0 63 V
0 1697 R
0 -63 V
2850 300 M
0 63 V
0 1697 R
0 -63 V
3150 300 M
0 63 V
0 1697 R
0 -63 V
3450 300 M
0 63 V
0 1697 R
0 -63 V
1.000 UL
LTb
450 300 M
3000 0 V
0 1760 V
-3000 0 V
450 300 L
1.000 UL
LT0
1590 510 M
-90 210 V
42 -54 R
-42 54 V
9 -68 V
1.000 UL
LT0
1740 510 M
120 210 V
-19 -71 R
19 71 V
-52 -52 V
1.000 UL
LT0
3087 1947 M
263 0 V
452 688 M
3 14 V
3 5 V
3 68 V
3 -58 V
3 52 V
3 -60 V
3 23 V
3 0 V
3 -60 V
3 108 V
3 -57 V
3 25 V
3 8 V
3 1 V
3 -87 V
3 94 V
3 68 V
3 -105 V
3 57 V
3 -34 V
3 17 V
3 86 V
3 -91 V
3 -7 V
3 -9 V
3 44 V
3 77 V
3 -43 V
3 0 V
3 -23 V
3 142 V
3 -110 V
3 -14 V
3 67 V
3 -56 V
3 -22 V
3 17 V
3 -62 V
3 139 V
3 -89 V
3 51 V
3 -6 V
3 -50 V
3 76 V
3 -66 V
3 110 V
3 -174 V
3 44 V
3 97 V
3 -128 V
3 70 V
3 -6 V
3 27 V
3 -37 V
3 -36 V
3 79 V
3 205 V
3 -348 V
3 263 V
3 -162 V
3 69 V
3 16 V
3 -105 V
3 98 V
3 -15 V
3 -13 V
3 126 V
3 -3 V
3 -6 V
3 -33 V
3 -31 V
3 -106 V
3 -110 V
3 181 V
3 133 V
3 59 V
3 -234 V
3 25 V
3 -19 V
3 91 V
3 -107 V
3 160 V
3 45 V
3 -176 V
3 338 V
3 -80 V
3 -230 V
3 65 V
3 158 V
3 -72 V
3 -46 V
3 134 V
3 -8 V
3 -139 V
3 -98 V
3 154 V
3 96 V
3 -103 V
3 93 V
3 -240 V
3 165 V
3 -238 V
3 482 V
3 -179 V
3 -145 V
3 38 V
3 -31 V
3 131 V
3 -121 V
3 170 V
3 -110 V
3 128 V
3 -166 V
3 143 V
3 61 V
3 -128 V
3 142 V
3 21 V
3 21 V
3 -222 V
3 17 V
3 9 V
3 66 V
3 -47 V
3 -265 V
3 297 V
3 95 V
3 35 V
3 -9 V
3 -42 V
3 -115 V
3 46 V
3 -38 V
3 81 V
3 -173 V
3 78 V
3 105 V
3 49 V
3 49 V
3 -225 V
3 52 V
3 -23 V
3 12 V
3 51 V
3 -6 V
3 95 V
3 27 V
3 -107 V
3 69 V
3 -84 V
3 -83 V
3 49 V
3 -104 V
3 -67 V
3 92 V
3 38 V
3 -128 V
3 182 V
3 34 V
3 -231 V
3 244 V
3 11 V
3 -104 V
3 -11 V
3 241 V
3 -125 V
3 -99 V
3 46 V
3 168 V
3 -174 V
3 27 V
3 26 V
3 38 V
3 -1 V
3 11 V
3 -30 V
3 -48 V
3 -28 V
3 158 V
3 -37 V
3 -138 V
3 -97 V
3 -56 V
3 182 V
3 -63 V
3 -80 V
3 44 V
3 47 V
3 -47 V
3 68 V
3 -159 V
3 137 V
3 -39 V
3 60 V
3 -82 V
3 140 V
3 -59 V
3 34 V
3 60 V
3 -123 V
3 190 V
3 -39 V
3 -141 V
3 -67 V
3 -79 V
3 226 V
3 -29 V
3 38 V
3 -139 V
3 258 V
3 -61 V
3 -95 V
3 -148 V
3 231 V
3 -37 V
3 106 V
3 -17 V
3 -101 V
3 -80 V
3 61 V
3 20 V
3 -56 V
3 -39 V
3 139 V
3 -167 V
3 63 V
3 227 V
3 -151 V
3 84 V
3 25 V
3 77 V
3 181 V
3 -404 V
3 -131 V
3 35 V
3 -81 V
3 -30 V
3 148 V
3 62 V
3 81 V
3 -38 V
3 2 V
3 236 V
3 -419 V
3 109 V
3 2 V
3 13 V
3 -26 V
3 -209 V
3 269 V
3 86 V
3 147 V
3 -4 V
3 -180 V
3 11 V
3 -30 V
3 -217 V
3 8 V
3 36 V
3 86 V
3 67 V
3 -75 V
3 33 V
3 -30 V
3 -83 V
3 122 V
3 -109 V
3 -47 V
3 167 V
3 -44 V
3 51 V
3 118 V
3 -54 V
3 -86 V
3 -20 V
3 44 V
3 -71 V
3 -27 V
3 213 V
3 130 V
3 -320 V
3 176 V
3 -137 V
3 -14 V
3 66 V
3 119 V
3 47 V
3 -133 V
3 123 V
3 -190 V
3 37 V
3 -165 V
3 311 V
3 -283 V
3 42 V
3 173 V
3 -253 V
3 230 V
3 -81 V
3 126 V
3 -182 V
3 -69 V
3 -14 V
3 148 V
3 -41 V
3 43 V
3 -2 V
3 -39 V
3 -20 V
3 115 V
3 -103 V
3 -32 V
3 31 V
3 69 V
3 118 V
3 50 V
3 53 V
3 -222 V
3 -70 V
3 59 V
3 54 V
3 -430 V
3 7 V
3 16 V
3 34 V
3 -2 V
3 -1 V
3 -10 V
3 11 V
3 9 V
3 18 V
3 22 V
3 -31 V
3 47 V
3 -25 V
3 17 V
3 10 V
3 -32 V
3 74 V
3 -27 V
3 18 V
3 -30 V
3 79 V
3 -83 V
3 -84 V
3 228 V
3 -64 V
3 34 V
3 27 V
3 82 V
3 -129 V
3 37 V
3 77 V
3 -119 V
3 156 V
3 15 V
3 -154 V
3 182 V
3 -64 V
3 22 V
3 -132 V
3 77 V
3 -48 V
3 -94 V
3 136 V
3 92 V
3 -438 V
3 410 V
3 -17 V
3 22 V
3 -9 V
3 -34 V
3 76 V
3 -133 V
3 92 V
3 59 V
3 -102 V
3 -227 V
3 239 V
3 108 V
3 -9 V
3 -94 V
3 138 V
3 -173 V
3 105 V
3 -108 V
3 219 V
3 42 V
3 -154 V
3 16 V
3 53 V
3 -31 V
3 -133 V
3 -20 V
3 178 V
3 -77 V
3 -95 V
currentpoint stroke M
3 453 V
3 -433 V
3 2 V
3 120 V
3 -58 V
3 -186 V
3 52 V
3 183 V
3 18 V
3 55 V
3 -51 V
3 61 V
3 -324 V
3 11 V
3 -58 V
3 126 V
3 1 V
3 35 V
3 -85 V
3 82 V
3 93 V
3 76 V
3 -120 V
3 82 V
3 -173 V
3 161 V
3 -3 V
3 251 V
3 -413 V
3 120 V
3 -43 V
3 201 V
3 -235 V
3 -136 V
3 335 V
3 -123 V
3 -94 V
3 17 V
3 56 V
3 -7 V
3 215 V
3 -362 V
3 45 V
3 53 V
3 3 V
3 25 V
3 -144 V
3 189 V
3 -37 V
3 -164 V
3 -317 V
3 302 V
3 205 V
3 18 V
3 -97 V
3 136 V
3 -108 V
3 1 V
3 -187 V
3 142 V
3 57 V
3 94 V
3 -187 V
3 125 V
3 86 V
3 -105 V
3 -20 V
3 263 V
3 -585 V
3 5 V
3 5 V
3 18 V
3 2 V
3 -32 V
3 38 V
3 29 V
3 -5 V
3 5 V
3 -106 V
3 67 V
3 21 V
3 24 V
3 4 V
3 17 V
3 28 V
3 -71 V
3 79 V
3 0 V
3 -59 V
3 69 V
3 5 V
3 -12 V
3 -25 V
3 0 V
3 111 V
3 28 V
3 -162 V
3 117 V
3 17 V
3 52 V
3 -5 V
3 28 V
3 -77 V
3 -65 V
3 -11 V
3 115 V
3 -151 V
3 151 V
3 15 V
3 98 V
3 -140 V
3 6 V
3 -24 V
3 272 V
3 -138 V
3 -42 V
3 114 V
3 -62 V
3 -59 V
3 78 V
3 -89 V
3 46 V
3 22 V
3 27 V
3 35 V
3 -40 V
3 64 V
3 45 V
3 -327 V
3 285 V
3 70 V
3 -114 V
3 -55 V
3 37 V
3 25 V
3 -32 V
3 130 V
3 -152 V
3 14 V
3 -81 V
3 24 V
3 47 V
3 -94 V
3 135 V
3 12 V
3 83 V
3 -86 V
3 24 V
3 74 V
3 24 V
3 -65 V
3 173 V
3 -383 V
3 285 V
3 -18 V
3 -117 V
3 -25 V
3 -33 V
3 8 V
3 94 V
3 -104 V
3 -1 V
3 135 V
3 -196 V
3 56 V
3 -82 V
3 -143 V
3 251 V
3 -91 V
3 26 V
3 -27 V
3 153 V
3 -165 V
3 9 V
3 69 V
3 -79 V
3 -26 V
3 91 V
3 163 V
3 115 V
3 -291 V
3 143 V
3 3 V
3 50 V
3 -25 V
3 58 V
3 -112 V
3 -43 V
3 232 V
3 -67 V
3 -112 V
3 13 V
3 -5 V
3 1 V
3 5 V
3 -179 V
3 123 V
3 34 V
3 182 V
3 70 V
3 -157 V
3 -37 V
3 -61 V
3 -94 V
1 105 R
3 132 V
3 -301 V
3 69 V
3 409 V
3 -426 V
3 12 V
3 189 V
3 -16 V
3 -149 V
3 152 V
3 -155 V
3 -27 V
3 136 V
3 -158 V
3 81 V
3 137 V
3 -43 V
3 161 V
3 -185 V
3 100 V
3 -9 V
3 -116 V
3 4 V
3 30 V
3 40 V
3 -36 V
3 -24 V
3 -68 V
3 101 V
3 -162 V
3 123 V
3 19 V
3 112 V
3 -148 V
3 -38 V
3 -27 V
3 77 V
3 41 V
3 -118 V
3 -52 V
3 105 V
3 85 V
3 -137 V
3 99 V
3 -176 V
3 155 V
3 -39 V
3 -22 V
3 198 V
3 -258 V
3 -3 V
3 43 V
3 -123 V
3 184 V
3 46 V
3 -39 V
3 4 V
3 -419 V
3 308 V
3 -28 V
3 119 V
3 47 V
3 -39 V
3 -130 V
3 151 V
3 -70 V
3 14 V
3 77 V
3 -73 V
3 -409 V
3 271 V
3 159 V
3 69 V
3 -145 V
3 -136 V
3 7 V
3 -4 V
3 52 V
3 -31 V
3 -47 V
3 120 V
3 -58 V
3 -43 V
3 95 V
3 -10 V
3 -139 V
3 -137 V
3 245 V
3 162 V
3 -78 V
3 -36 V
3 22 V
3 -159 V
3 101 V
3 75 V
3 96 V
3 -144 V
3 200 V
3 -108 V
3 78 V
3 1 V
3 -2 V
3 -21 V
3 -49 V
3 42 V
3 -12 V
3 -126 V
3 312 V
3 -237 V
3 -52 V
3 4 V
3 81 V
3 4 V
3 -196 V
3 59 V
3 58 V
3 173 V
3 -79 V
3 16 V
3 -62 V
3 -162 V
3 133 V
3 -78 V
3 124 V
3 68 V
3 -79 V
3 48 V
3 -149 V
3 83 V
3 5 V
3 -45 V
3 46 V
3 -123 V
3 -123 V
3 -96 V
3 119 V
3 253 V
3 -87 V
3 241 V
3 -159 V
3 89 V
3 175 V
3 -232 V
3 -111 V
3 397 V
3 -501 V
3 61 V
3 -20 V
3 2 V
3 -6 V
3 -16 V
3 -10 V
3 100 V
3 -66 V
3 -111 V
3 195 V
3 -33 V
3 -45 V
3 1 V
3 27 V
3 38 V
3 -6 V
3 52 V
3 -19 V
3 53 V
3 -188 V
3 -12 V
3 111 V
3 -54 V
3 51 V
3 25 V
3 -21 V
3 66 V
3 181 V
3 -30 V
3 -283 V
3 261 V
3 24 V
3 -54 V
3 135 V
3 73 V
3 -401 V
3 15 V
3 2 V
3 -134 V
3 116 V
3 163 V
3 -104 V
3 124 V
3 -154 V
3 230 V
3 -309 V
3 -35 V
3 343 V
3 -306 V
currentpoint stroke M
3 10 V
3 -9 V
3 73 V
3 -99 V
3 -196 V
3 281 V
3 37 V
3 -79 V
3 87 V
3 -98 V
3 105 V
3 -62 V
3 -45 V
3 240 V
3 -227 V
3 79 V
3 9 V
3 -207 V
3 135 V
3 185 V
3 -82 V
3 -356 V
3 270 V
3 -10 V
3 -93 V
3 140 V
3 73 V
3 -130 V
3 165 V
3 -82 V
3 -110 V
3 -69 V
3 169 V
3 -177 V
3 109 V
3 92 V
3 -117 V
3 189 V
3 -44 V
3 29 V
3 -118 V
3 120 V
3 -40 V
3 206 V
3 -378 V
3 -18 V
3 118 V
3 46 V
3 -148 V
3 -106 V
3 165 V
3 23 V
3 142 V
3 -144 V
3 142 V
3 21 V
3 -85 V
3 63 V
3 -108 V
3 -55 V
3 -137 V
3 -73 V
3 -11 V
3 302 V
3 -150 V
3 89 V
3 -17 V
3 -86 V
3 14 V
3 165 V
3 -153 V
3 198 V
3 52 V
3 37 V
3 -37 V
3 -24 V
3 72 V
3 -271 V
3 -71 V
3 450 V
3 -487 V
3 34 V
3 -98 V
3 117 V
3 12 V
3 -9 V
3 19 V
3 52 V
3 48 V
3 -231 V
3 -123 V
3 424 V
3 -62 V
3 -57 V
3 -70 V
3 6 V
3 -328 V
3 341 V
3 -30 V
3 -34 V
3 46 V
3 26 V
3 -15 V
3 31 V
3 -28 V
3 153 V
3 -142 V
3 75 V
3 -146 V
3 -1 V
3 211 V
3 21 V
3 -133 V
3 136 V
3 75 V
3 -213 V
3 85 V
3 45 V
3 -18 V
3 -100 V
3 204 V
3 38 V
3 57 V
3 -137 V
3 -41 V
3 34 V
3 -39 V
3 -47 V
3 49 V
3 -17 V
3 58 V
3 -90 V
3 85 V
3 -224 V
3 188 V
3 -89 V
3 105 V
3 139 V
3 -142 V
3 58 V
3 43 V
3 -5 V
3 -265 V
3 72 V
3 27 V
3 -136 V
3 154 V
3 7 V
3 -69 V
3 -78 V
3 48 V
3 93 V
3 162 V
3 -243 V
3 171 V
3 -214 V
3 -18 V
3 372 V
3 -257 V
3 16 V
3 29 V
3 -6 V
3 -8 V
3 125 V
3 -113 V
3 89 V
3 -185 V
3 250 V
3 -184 V
3 243 V
3 -143 V
3 19 V
3 -145 V
3 85 V
3 -52 V
3 -2 V
3 114 V
3 -29 V
3 -160 V
3 148 V
3 -94 V
3 15 V
3 31 V
3 -202 V
3 108 V
3 -48 V
3 75 V
3 -70 V
3 24 V
3 11 V
3 -46 V
3 158 V
3 -98 V
3 -229 V
3 257 V
3 96 V
3 -17 V
3 -185 V
3 186 V
3 -151 V
3 175 V
3 -62 V
3 68 V
1.000 UL
LT1
3087 1847 M
263 0 V
452 1119 M
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
31 0 V
30 0 V
30 0 V
30 0 V
31 0 V
30 0 V
stroke
grestore
end
showpage
}}%
\put(3037,1847){\makebox(0,0)[r]{Geometric mean, $p=7.3$}}%
\put(3037,1947){\makebox(0,0)[r]{$N=100$, $\sigma_\epsilon=0.10$}}%
\put(1665,432){\makebox(0,0){Crashes}}%
\put(600,1972){\makebox(0,0){(a)}}%
\put(1950,50){\makebox(0,0){Time $t$}}%
\put(100,1180){%
\special{ps: gsave currentpoint currentpoint translate
270 rotate neg exch neg exch translate}%
\makebox(0,0)[b]{\shortstack{Price $p_t$}}%
\special{ps: currentpoint grestore moveto}%
}%
\put(3450,200){\makebox(0,0){2000}}%
\put(3150,200){\makebox(0,0){1800}}%
\put(2850,200){\makebox(0,0){1600}}%
\put(2550,200){\makebox(0,0){1400}}%
\put(2250,200){\makebox(0,0){1200}}%
\put(1950,200){\makebox(0,0){1000}}%
\put(1650,200){\makebox(0,0){800}}%
\put(1350,200){\makebox(0,0){600}}%
\put(1050,200){\makebox(0,0){400}}%
\put(750,200){\makebox(0,0){200}}%
\put(450,200){\makebox(0,0){0}}%
\put(400,2060){\makebox(0,0)[r]{1000}}%
\put(400,1620){\makebox(0,0)[r]{100}}%
\put(400,1180){\makebox(0,0)[r]{10}}%
\put(400,740){\makebox(0,0)[r]{1}}%
\put(400,300){\makebox(0,0)[r]{0.1}}%
\end{picture}%
\endgroup
\endinput


==> chResults2/csemCrashes0.15.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup%
  \makeatletter%
  \newcommand{\GNUPLOTspecial}{%
    \@sanitize\catcode`\%=14\relax\special}%
  \setlength{\unitlength}{0.1bp}%
{\GNUPLOTspecial{!
%!PS-Adobe-2.0 EPSF-2.0
%%Title: csemCrashes0.15.tex
%%Creator: gnuplot 3.7 patchlevel 1
%%CreationDate: Fri Jun 09 21:32:07 2000
%%DocumentFonts: 
%%BoundingBox: 0 0 360 216
%%Orientation: Landscape
%%EndComments
/gnudict 256 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/vshift -33 def
/dl {10 mul} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/UP { dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke userlinewidth 2 mul setlinewidth } def
/AL { stroke userlinewidth 2 div setlinewidth } def
/UL { dup gnulinewidth mul /userlinewidth exch def
      10 mul /udl exch def } def
/PL { stroke userlinewidth setlinewidth } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 udl mul 2 udl mul] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 1 0 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 1 0 DL } def
/LT2 { PL [2 dl 3 dl] 0 0 1 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/Pnt { stroke [] 0 setdash
   gsave 1 setlinecap M 0 0 V stroke grestore } def
/Dia { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt } def
/Pls { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/Box { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt } def
/Crs { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/TriU { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt  } def
/Star { 2 copy Pls Crs } def
/BoxF { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V  hpt2 0 V  0 vpt2 V
  hpt2 neg 0 V  closepath fill } def
/TriUF { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill } def
/TriD { stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt  } def
/TriDF { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill } def
/Pent { stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt } def
/PentF { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore } def
/Circle { stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt } def
/CircleF { stroke [] 0 setdash hpt 0 360 arc fill } def
/C0 { BL [] 0 setdash 2 copy moveto vpt 90 450  arc } bind def
/C1 { BL [] 0 setdash 2 copy        moveto
       2 copy  vpt 0 90 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C2 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C3 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C4 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C5 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 90 arc
       2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc } bind def
/C6 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 90 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C7 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 0 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C8 { BL [] 0 setdash 2 copy moveto
      2 copy vpt 270 360 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C9 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 270 450 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C10 { BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
       2 copy moveto
       2 copy vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C11 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
       2 copy moveto
       2 copy  vpt 270 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C12 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C13 { BL [] 0 setdash  2 copy moveto
       2 copy  vpt 0 90 arc closepath fill
       2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C14 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 360 arc closepath fill
               vpt 0 360 arc } bind def
/C15 { BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/Rec   { newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
       neg 0 rlineto closepath } bind def
/Square { dup Rec } bind def
/Bsquare { vpt sub exch vpt sub exch vpt2 Square } bind def
/S0 { BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare } bind def
/S1 { BL [] 0 setdash 2 copy vpt Square fill Bsquare } bind def
/S2 { BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S3 { BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare } bind def
/S4 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S5 { BL [] 0 setdash 2 copy 2 copy vpt Square fill
       exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S6 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S7 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
       2 copy vpt Square fill
       Bsquare } bind def
/S8 { BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare } bind def
/S9 { BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S10 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
       Bsquare } bind def
/S11 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
       Bsquare } bind def
/S12 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare } bind def
/S13 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy vpt Square fill Bsquare } bind def
/S14 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S15 { BL [] 0 setdash 2 copy Bsquare fill Bsquare } bind def
/D0 { gsave translate 45 rotate 0 0 S0 stroke grestore } bind def
/D1 { gsave translate 45 rotate 0 0 S1 stroke grestore } bind def
/D2 { gsave translate 45 rotate 0 0 S2 stroke grestore } bind def
/D3 { gsave translate 45 rotate 0 0 S3 stroke grestore } bind def
/D4 { gsave translate 45 rotate 0 0 S4 stroke grestore } bind def
/D5 { gsave translate 45 rotate 0 0 S5 stroke grestore } bind def
/D6 { gsave translate 45 rotate 0 0 S6 stroke grestore } bind def
/D7 { gsave translate 45 rotate 0 0 S7 stroke grestore } bind def
/D8 { gsave translate 45 rotate 0 0 S8 stroke grestore } bind def
/D9 { gsave translate 45 rotate 0 0 S9 stroke grestore } bind def
/D10 { gsave translate 45 rotate 0 0 S10 stroke grestore } bind def
/D11 { gsave translate 45 rotate 0 0 S11 stroke grestore } bind def
/D12 { gsave translate 45 rotate 0 0 S12 stroke grestore } bind def
/D13 { gsave translate 45 rotate 0 0 S13 stroke grestore } bind def
/D14 { gsave translate 45 rotate 0 0 S14 stroke grestore } bind def
/D15 { gsave translate 45 rotate 0 0 S15 stroke grestore } bind def
/DiaE { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke } def
/BoxE { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke } def
/TriUE { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke } def
/TriDE { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke } def
/PentE { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore } def
/CircE { stroke [] 0 setdash 
  hpt 0 360 arc stroke } def
/Opaque { gsave closepath 1 setgray fill grestore 0 setgray closepath } def
/DiaW { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke } def
/BoxW { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke } def
/TriUW { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke } def
/TriDW { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke } def
/PentW { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore } def
/CircW { stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke } def
/BoxFill { gsave Rec 1 setgray fill grestore } def
end
%%EndProlog
}}%
\begin{picture}(3600,2160)(0,0)%
{\GNUPLOTspecial{"
gnudict begin
gsave
0 0 translate
0.100 0.100 scale
0 setgray
newpath
1.000 UL
LTb
400 300 M
63 0 V
2987 0 R
-63 0 V
400 477 M
31 0 V
3019 0 R
-31 0 V
400 580 M
31 0 V
3019 0 R
-31 0 V
400 653 M
31 0 V
3019 0 R
-31 0 V
400 710 M
31 0 V
3019 0 R
-31 0 V
400 757 M
31 0 V
3019 0 R
-31 0 V
400 796 M
31 0 V
3019 0 R
-31 0 V
400 830 M
31 0 V
3019 0 R
-31 0 V
400 860 M
31 0 V
3019 0 R
-31 0 V
400 887 M
63 0 V
2987 0 R
-63 0 V
400 1063 M
31 0 V
3019 0 R
-31 0 V
400 1167 M
31 0 V
3019 0 R
-31 0 V
400 1240 M
31 0 V
3019 0 R
-31 0 V
400 1297 M
31 0 V
3019 0 R
-31 0 V
400 1343 M
31 0 V
3019 0 R
-31 0 V
400 1382 M
31 0 V
3019 0 R
-31 0 V
400 1416 M
31 0 V
3019 0 R
-31 0 V
400 1446 M
31 0 V
3019 0 R
-31 0 V
400 1473 M
63 0 V
2987 0 R
-63 0 V
400 1650 M
31 0 V
3019 0 R
-31 0 V
400 1753 M
31 0 V
3019 0 R
-31 0 V
400 1827 M
31 0 V
3019 0 R
-31 0 V
400 1883 M
31 0 V
3019 0 R
-31 0 V
400 1930 M
31 0 V
3019 0 R
-31 0 V
400 1969 M
31 0 V
3019 0 R
-31 0 V
400 2003 M
31 0 V
3019 0 R
-31 0 V
400 2033 M
31 0 V
3019 0 R
-31 0 V
400 2060 M
63 0 V
2987 0 R
-63 0 V
400 300 M
0 63 V
0 1697 R
0 -63 V
705 300 M
0 63 V
0 1697 R
0 -63 V
1010 300 M
0 63 V
0 1697 R
0 -63 V
1315 300 M
0 63 V
0 1697 R
0 -63 V
1620 300 M
0 63 V
0 1697 R
0 -63 V
1925 300 M
0 63 V
0 1697 R
0 -63 V
2230 300 M
0 63 V
0 1697 R
0 -63 V
2535 300 M
0 63 V
0 1697 R
0 -63 V
2840 300 M
0 63 V
0 1697 R
0 -63 V
3145 300 M
0 63 V
0 1697 R
0 -63 V
3450 300 M
0 63 V
0 1697 R
0 -63 V
1.000 UL
LTb
400 300 M
3050 0 V
0 1760 V
-3050 0 V
400 300 L
1.000 UL
LT0
3087 1947 M
263 0 V
402 735 M
3 110 V
3 -2 V
3 4 V
3 -31 V
3 22 V
3 -51 V
3 92 V
3 117 V
3 -127 V
3 -45 V
3 119 V
3 -355 V
3 384 V
3 -95 V
3 106 V
3 11 V
3 -13 V
3 -6 V
3 41 V
4 -243 V
3 230 V
3 31 V
3 -19 V
3 30 V
3 -101 V
3 -151 V
3 83 V
3 -15 V
3 98 V
3 -81 V
3 89 V
3 80 V
3 -72 V
3 -109 V
3 117 V
3 -74 V
3 51 V
3 124 V
3 62 V
4 -200 V
3 35 V
3 56 V
3 207 V
3 -266 V
3 -23 V
3 247 V
3 -148 V
3 86 V
3 96 V
3 -166 V
3 94 V
3 -124 V
3 83 V
3 179 V
3 -163 V
3 -103 V
3 -134 V
3 280 V
3 -33 V
4 -151 V
3 20 V
3 105 V
3 158 V
3 -121 V
3 -141 V
3 67 V
3 -1 V
3 -171 V
3 104 V
3 -107 V
3 163 V
3 -82 V
3 -15 V
3 -105 V
3 96 V
3 59 V
3 17 V
3 -71 V
3 85 V
4 -170 V
3 96 V
3 83 V
3 40 V
3 -224 V
3 260 V
3 -94 V
3 -148 V
3 190 V
3 -4 V
3 -78 V
3 -85 V
3 161 V
3 6 V
3 80 V
3 -43 V
3 -35 V
3 -59 V
3 61 V
3 -21 V
4 -114 V
3 4 V
3 1 V
3 -109 V
3 45 V
3 61 V
3 152 V
3 -115 V
3 17 V
3 -18 V
3 27 V
3 5 V
3 72 V
3 -191 V
3 195 V
3 -11 V
3 -119 V
3 -139 V
3 300 V
3 -234 V
4 216 V
3 -190 V
3 197 V
3 -106 V
3 -37 V
3 104 V
3 -18 V
3 75 V
3 -54 V
3 -142 V
3 68 V
3 76 V
3 9 V
3 -17 V
3 -12 V
3 -153 V
3 49 V
3 -37 V
3 214 V
3 -50 V
4 -68 V
3 61 V
3 -31 V
3 -252 V
3 239 V
3 -50 V
3 123 V
3 4 V
3 -58 V
3 -33 V
3 260 V
3 -309 V
3 45 V
3 230 V
3 12 V
3 -101 V
3 46 V
3 -152 V
3 100 V
3 -132 V
4 112 V
3 -11 V
3 35 V
3 -3 V
3 44 V
3 -146 V
3 34 V
3 86 V
3 -67 V
3 -10 V
3 118 V
3 -66 V
3 -133 V
3 328 V
3 -346 V
3 50 V
3 58 V
3 116 V
3 -158 V
3 73 V
4 -78 V
3 -23 V
3 328 V
3 -79 V
3 -144 V
3 25 V
3 -18 V
3 89 V
3 -101 V
3 54 V
3 -135 V
3 152 V
3 -226 V
3 10 V
3 195 V
3 -210 V
3 42 V
3 284 V
3 -83 V
3 6 V
4 -48 V
3 33 V
3 -78 V
3 297 V
3 -160 V
3 -117 V
3 -87 V
3 134 V
3 -65 V
3 -222 V
3 336 V
3 -210 V
3 147 V
3 55 V
3 -85 V
3 -107 V
3 82 V
3 140 V
3 7 V
3 -50 V
4 13 V
3 -74 V
3 -194 V
3 -60 V
3 235 V
3 -78 V
3 -62 V
3 -88 V
3 372 V
3 -218 V
3 71 V
3 63 V
3 -201 V
3 66 V
3 98 V
3 28 V
3 -23 V
3 -146 V
3 -31 V
3 73 V
4 61 V
3 -82 V
3 -197 V
3 154 V
3 12 V
3 102 V
3 -58 V
3 -35 V
3 -29 V
3 11 V
3 99 V
3 -246 V
3 126 V
3 -63 V
3 225 V
3 -95 V
3 -66 V
3 133 V
3 -133 V
3 -50 V
4 -14 V
3 62 V
3 65 V
3 38 V
3 -29 V
3 137 V
3 -272 V
3 273 V
3 -331 V
3 339 V
3 -212 V
3 247 V
3 -36 V
3 -64 V
3 65 V
3 -185 V
3 180 V
3 -111 V
3 -22 V
3 -54 V
4 -22 V
3 80 V
3 -21 V
3 66 V
3 12 V
3 -32 V
3 -117 V
3 184 V
3 -61 V
3 -94 V
3 -43 V
3 299 V
3 -297 V
3 266 V
3 -82 V
3 87 V
3 -272 V
3 312 V
3 -363 V
3 148 V
4 96 V
3 7 V
3 21 V
3 79 V
3 -144 V
3 -52 V
3 -87 V
3 43 V
3 190 V
3 75 V
3 -140 V
3 -135 V
3 126 V
3 115 V
3 -237 V
3 -16 V
3 9 V
3 45 V
3 92 V
3 -99 V
4 112 V
3 -130 V
3 26 V
3 -20 V
3 190 V
3 -133 V
3 43 V
3 -9 V
3 57 V
3 -143 V
3 191 V
3 -165 V
3 94 V
3 -141 V
3 105 V
3 -145 V
3 94 V
3 14 V
3 12 V
3 -119 V
4 177 V
3 -136 V
3 56 V
3 7 V
3 -83 V
3 118 V
3 0 V
3 -37 V
3 37 V
3 6 V
3 13 V
3 -138 V
3 -19 V
3 161 V
3 7 V
3 86 V
3 -442 V
3 221 V
3 -126 V
3 134 V
4 68 V
3 -122 V
3 -35 V
3 27 V
3 154 V
3 38 V
3 -36 V
3 -18 V
3 -59 V
3 -15 V
3 96 V
3 -122 V
3 -1 V
3 13 V
3 1 V
3 110 V
3 -61 V
3 69 V
3 -125 V
3 62 V
4 -45 V
3 25 V
3 92 V
3 -92 V
3 13 V
3 44 V
3 67 V
3 -199 V
3 -7 V
3 97 V
3 -330 V
3 543 V
3 -284 V
3 235 V
3 -157 V
3 -12 V
3 7 V
3 147 V
currentpoint stroke M
3 -177 V
3 22 V
4 44 V
3 16 V
3 -16 V
3 -44 V
3 26 V
3 -37 V
3 32 V
3 -4 V
3 -16 V
3 -43 V
3 182 V
3 -99 V
3 -20 V
3 -55 V
3 308 V
3 -269 V
3 -11 V
3 -44 V
3 61 V
3 31 V
4 161 V
3 -250 V
3 -100 V
3 50 V
3 152 V
3 -129 V
3 125 V
3 55 V
3 -59 V
3 -103 V
3 29 V
3 80 V
3 -117 V
3 155 V
3 -4 V
3 28 V
3 -175 V
3 213 V
3 -89 V
3 -39 V
4 -57 V
3 134 V
3 -94 V
3 -44 V
3 -137 V
3 290 V
3 -103 V
3 -15 V
3 233 V
3 -188 V
3 -117 V
3 67 V
3 31 V
3 -53 V
3 -14 V
3 127 V
3 -49 V
3 -31 V
3 170 V
3 -128 V
4 -128 V
3 -39 V
3 -100 V
3 326 V
3 70 V
3 -70 V
3 39 V
3 -120 V
3 47 V
3 -72 V
3 69 V
3 -107 V
3 -79 V
3 323 V
3 -67 V
3 153 V
3 -276 V
3 79 V
3 61 V
3 -133 V
4 194 V
3 -108 V
3 3 V
3 -242 V
3 263 V
3 -122 V
3 147 V
3 -86 V
3 -231 V
3 246 V
3 84 V
3 -187 V
3 4 V
3 158 V
3 -70 V
3 -33 V
3 156 V
3 -306 V
3 163 V
3 -21 V
4 14 V
3 22 V
3 10 V
3 -36 V
3 -157 V
3 138 V
3 -174 V
3 176 V
3 68 V
3 -7 V
3 31 V
3 -143 V
3 28 V
3 23 V
3 104 V
3 -111 V
3 122 V
3 -244 V
3 168 V
3 138 V
4 -176 V
3 -34 V
3 -161 V
3 336 V
3 94 V
3 -214 V
3 51 V
3 -72 V
3 -37 V
3 -64 V
3 133 V
3 -148 V
3 19 V
3 198 V
3 -211 V
3 173 V
3 -36 V
3 -242 V
3 102 V
3 17 V
4 31 V
3 -23 V
3 157 V
3 -56 V
3 144 V
3 -97 V
3 -231 V
3 80 V
3 61 V
3 -76 V
3 9 V
3 -29 V
3 19 V
3 8 V
3 190 V
3 -248 V
3 360 V
3 -351 V
3 211 V
3 -3 V
4 -104 V
3 20 V
3 113 V
3 -15 V
3 -8 V
3 -73 V
3 69 V
3 -80 V
3 -228 V
3 174 V
3 -128 V
3 324 V
3 35 V
3 31 V
3 -101 V
3 56 V
3 -211 V
3 276 V
3 -92 V
3 -114 V
4 110 V
3 -34 V
3 -60 V
3 26 V
3 240 V
3 -106 V
3 -10 V
3 17 V
3 -208 V
3 -141 V
3 229 V
3 67 V
3 -57 V
3 -128 V
3 -10 V
3 112 V
3 -100 V
3 43 V
3 -97 V
3 104 V
4 -61 V
3 -35 V
3 201 V
3 -237 V
3 240 V
3 -13 V
3 -111 V
3 -89 V
3 154 V
3 112 V
3 -194 V
3 84 V
3 -3 V
3 -177 V
3 75 V
3 122 V
3 -50 V
3 -151 V
3 119 V
3 134 V
4 -132 V
3 65 V
3 25 V
3 -285 V
3 107 V
3 130 V
3 25 V
3 -131 V
3 -30 V
3 107 V
3 72 V
3 52 V
3 -136 V
3 81 V
3 -45 V
3 22 V
3 -158 V
3 135 V
3 194 V
3 -18 V
4 -198 V
3 252 V
3 -320 V
3 -28 V
3 197 V
3 -123 V
3 -165 V
3 258 V
3 -3 V
3 137 V
3 -140 V
3 -40 V
3 86 V
3 -175 V
3 145 V
3 -4 V
3 -94 V
3 100 V
3 -102 V
3 -118 V
4 -41 V
3 257 V
3 64 V
3 -177 V
3 -73 V
3 142 V
3 105 V
3 47 V
3 -102 V
3 52 V
3 -124 V
3 143 V
3 -185 V
3 -141 V
3 44 V
3 101 V
3 -69 V
3 148 V
3 -164 V
3 287 V
4 -137 V
3 83 V
3 -3 V
3 -142 V
3 204 V
3 10 V
3 82 V
3 -228 V
3 70 V
3 -128 V
3 -62 V
3 181 V
3 -159 V
3 83 V
3 5 V
3 65 V
3 -77 V
3 -186 V
3 95 V
3 26 V
4 259 V
3 130 V
3 -98 V
3 -152 V
3 -218 V
3 290 V
3 -107 V
3 -16 V
3 234 V
3 -250 V
3 56 V
3 7 V
3 -114 V
3 56 V
3 18 V
3 416 V
3 -618 V
3 163 V
3 142 V
3 24 V
4 16 V
3 -105 V
3 71 V
3 0 V
3 -216 V
3 268 V
3 -121 V
3 -126 V
3 49 V
3 198 V
3 -222 V
3 4 V
3 94 V
3 -149 V
3 -4 V
3 -99 V
3 85 V
3 -15 V
3 380 V
3 -332 V
4 222 V
3 -93 V
3 -202 V
3 -22 V
3 108 V
3 -173 V
3 436 V
3 -148 V
3 -117 V
3 114 V
3 63 V
3 -77 V
3 -49 V
3 65 V
3 91 V
3 -189 V
3 127 V
3 -9 V
3 -209 V
3 -10 V
4 195 V
3 163 V
3 -177 V
3 9 V
3 -228 V
3 163 V
3 -177 V
3 247 V
3 -286 V
3 422 V
3 -422 V
3 445 V
3 -124 V
3 -23 V
3 -246 V
3 206 V
3 -19 V
2 100 R
3 -115 V
3 176 V
3 -405 V
3 384 V
3 -111 V
3 82 V
3 -133 V
3 133 V
3 -140 V
3 -97 V
3 192 V
3 -113 V
3 16 V
4 -18 V
3 42 V
3 -75 V
3 -2 V
3 -73 V
3 37 V
3 18 V
currentpoint stroke M
3 19 V
3 79 V
3 -86 V
3 -2 V
3 68 V
3 -333 V
3 378 V
3 -17 V
3 56 V
3 -106 V
3 42 V
3 -126 V
3 123 V
4 76 V
3 -313 V
3 248 V
3 -204 V
3 203 V
3 -88 V
3 37 V
3 -118 V
3 146 V
3 44 V
3 -331 V
3 112 V
3 178 V
3 73 V
3 -56 V
3 71 V
3 -237 V
3 -7 V
3 186 V
3 -91 V
4 61 V
3 23 V
3 -120 V
3 -21 V
3 -30 V
3 62 V
3 -68 V
3 -286 V
3 437 V
3 40 V
3 -168 V
3 46 V
3 44 V
3 -70 V
3 336 V
3 -274 V
3 27 V
3 -160 V
3 58 V
3 163 V
4 -85 V
3 92 V
3 135 V
3 -105 V
3 -249 V
3 211 V
3 -27 V
3 -62 V
3 -8 V
3 -182 V
3 260 V
3 -65 V
3 -18 V
3 67 V
3 220 V
3 -227 V
3 -54 V
3 196 V
3 -209 V
3 104 V
4 21 V
3 -89 V
3 129 V
3 -12 V
3 -181 V
3 358 V
3 -74 V
3 -89 V
3 -125 V
3 19 V
3 61 V
3 111 V
3 -205 V
3 47 V
3 -141 V
3 377 V
3 -385 V
3 219 V
3 -14 V
3 -75 V
4 33 V
3 -8 V
3 110 V
3 -295 V
3 293 V
3 -76 V
3 116 V
3 -76 V
3 -86 V
3 -67 V
3 150 V
3 -235 V
3 205 V
3 8 V
3 102 V
3 -33 V
3 -337 V
3 305 V
3 -252 V
3 181 V
4 -2 V
3 -157 V
3 48 V
3 114 V
3 -84 V
3 4 V
3 -40 V
3 78 V
3 139 V
3 -137 V
3 -67 V
3 183 V
3 58 V
3 -136 V
3 -69 V
3 70 V
3 -114 V
3 151 V
3 -105 V
3 -18 V
4 88 V
3 44 V
3 -326 V
3 232 V
3 -57 V
3 -38 V
3 174 V
3 -48 V
3 -76 V
3 -55 V
3 -16 V
3 125 V
3 -81 V
3 133 V
3 -98 V
3 15 V
3 80 V
3 -69 V
3 -16 V
3 164 V
4 -81 V
3 -151 V
3 134 V
3 -78 V
3 89 V
3 171 V
3 -349 V
3 22 V
3 66 V
3 111 V
3 -118 V
3 -63 V
3 161 V
3 -117 V
3 -67 V
3 -80 V
3 104 V
3 185 V
3 36 V
3 -196 V
4 63 V
3 -65 V
3 69 V
3 99 V
3 21 V
3 47 V
3 -198 V
3 -66 V
3 92 V
3 -57 V
3 77 V
3 -144 V
3 -212 V
3 410 V
3 -17 V
3 47 V
3 -8 V
3 -37 V
3 11 V
3 -223 V
4 65 V
3 44 V
3 -173 V
3 213 V
3 -114 V
3 356 V
3 -220 V
3 148 V
3 -254 V
3 146 V
1.000 UL
LT1
3087 1847 M
263 0 V
402 1097 M
30 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
31 0 V
31 0 V
30 0 V
31 0 V
31 0 V
stroke
grestore
end
showpage
}}%
\put(3037,1847){\makebox(0,0)[r]{Geometric mean, $p=2.3$}}%
\put(3037,1947){\makebox(0,0)[r]{$N=100$, $\sigma_\epsilon=0.15$}}%
\put(553,1972){\makebox(0,0){(b)}}%
\put(1925,50){\makebox(0,0){Time $t$}}%
\put(100,1180){%
\special{ps: gsave currentpoint currentpoint translate
270 rotate neg exch neg exch translate}%
\makebox(0,0)[b]{\shortstack{Price $p_t$}}%
\special{ps: currentpoint grestore moveto}%
}%
\put(3450,200){\makebox(0,0){2000}}%
\put(3145,200){\makebox(0,0){1800}}%
\put(2840,200){\makebox(0,0){1600}}%
\put(2535,200){\makebox(0,0){1400}}%
\put(2230,200){\makebox(0,0){1200}}%
\put(1925,200){\makebox(0,0){1000}}%
\put(1620,200){\makebox(0,0){800}}%
\put(1315,200){\makebox(0,0){600}}%
\put(1010,200){\makebox(0,0){400}}%
\put(705,200){\makebox(0,0){200}}%
\put(400,200){\makebox(0,0){0}}%
\put(350,2060){\makebox(0,0)[r]{100}}%
\put(350,1473){\makebox(0,0)[r]{10}}%
\put(350,887){\makebox(0,0)[r]{1}}%
\put(350,300){\makebox(0,0)[r]{0.1}}%
\end{picture}%
\endgroup
\endinput


==> chResults2/sectBubbles.tex <==
\section{Bubbles and crashes}

In this section we briefly look for the existence of price bubbles and crashes---sustained periods of over- and under-valuation of the stock \cite{arthur97}---in both CSEM and DSEM.  Market bubbles and crashes are thought to arise not from exogenous factors but via self-fulfilling ``prophecies'' of future price movements \cite{flood90, kraus98}.  (For instance, if enough investors believe a stock's price will decline and attempt to sell before it does, the resulting oversupply will indeed drive the price down.)

Bubbles and crashes are difficult to establish from market data because it can be difficult (impossible?) to factor out all the exogenous factors which may influence a stock's price.  Empirical markets are strongly coupled to all facets of human activities and are therefore poor experimental subjects.  Every significant movement in the markets is accompanied by a flood of media reports explaining why the movement occured---and since it is frequently difficult to quantify the suggested impulses, these explanations are beyond the scope of science to test.

In contrast, both market models presented in this thesis can be tested for endogenous bubbles and crashes because all exogenous factors have been explicitly formulated.  CSEM actually contains no external influences and the dynamics are completely a consequence of interactions between agents.  DSEM does have a single exogenous component, the news, but it is a simple scalar quantity directly related to the logarithm of the price as discussed in \sect{dsemPriceResponse}.

To identify bubbles and crashes it is necessary to determine the ``proper'' price for the stock.  (The term ``proper'' is used to distinguish this value from the ``fundamental'' price because in neither model does the stock have any fundamental value: agents only place a value on each share in the expectation of earning a profit.)  

\subsection{Centralized Stock Exchange Model}

As was observed in \fig{resultsCsemPhases}, the price tends to converge to a steady-state value in CSEM, so this is taken to be the ``proper'' price.  It is calculated by taking the (logarithmic) mean of the price over the series, neglecting the initial transient.

\begin{figure}\centering
% GnuPlot: "..\..\Generation 4\DataV2.2\csemCrashes0.10.plt"
% GnuPlot: "..\..\Generation 4\DataV2.2\csemCrashes0.15.plt"
	\input{chResults2/csemCrashes0.10.tex} \\
	\input{chResults2/csemCrashes0.15.tex}
	\caption{Below the critical point $\sigma_\epsilon\leq \sigma_c\approx 0.12$ (a) the price series exhibits extended ``crashes'' (periods when the price is unusually low) with slow recoveries not observed when $\sigma_\epsilon>\sigma_c$ (b).  The data come from CSEM Dataset 1 (\tbl{resultsCsemDataset1}).}
\label{fig:results2CsemCrashes}
\end{figure}

Bubbles are then defined, in CSEM, as periods when the price is above the proper price and crashes are periods when the price is below the proper price.  As can be seen in \fig{results2CsemCrashes} the price series contains occasional, large crashes when $\sigma_\epsilon$ is small, less than than $\sigma_c\approx 0.12$ but the existence of bubbles was not as clear.  When the crashes occur the recovery time can be quite long, on the order of a hundred trading days.  When the forecast error is above the critical point neither crashes nor bubbles are observed.

\subsection{Decentralized Stock Exchange Model}

In DSEM, the ``proper'' price does not converge to a constant but fluctuates with the news according to 
\begin{equation}
	\log p(t) = C \eta(t)
\end{equation}
where $\eta(t)$ is the cumulative news up to time $t$.  The proportionality constant $C$ is unknown so it is chosen in order to minimize the sum-of-squares deviation between the curves.  (The fits were determined to be of good quality by drawing scatter plots of $\log p / C \eta$ vs. $\eta$, revealing uniform statistical spread and no remaining correlations.)

\begin{figure}\centering
% GnuPlot: "..\..\Generation 7\DataV2.3\dsemBubblesCrashes.plt"
	\input{chResults2/dsemBubblesCrashes}
	\caption{Sustained bubbles and crashes are only observed near the critical point $r_p=1$ in DSEM.  Near the first-order transition $r_p\approx -0.33$ intermittent bursts are observed but the fluctuations are not systematically high or low.  The data come from DSEM Dataset 1 (\tbl{resultsDsemDataset1}).}
\label{fig:results2DsemBubblesCrashes}
\end{figure}

The ratio of the actual price to the ``proper'' price, shown in \fig{results2DsemBubblesCrashes}, was used as an indicator of bubbles and crashes.  Bubbles would be indicated by periods when the ratio was significantly greater than one and crashes by a period less than one.  No evidence was found except in the region of the critical point.  Although the fluctuations are large, some evidence of sustained deviations from the proper price is apparent in this region.  

Farther from the critical point the both the fluctuations and the systematic deviations diminish until the first order transition near $r_2\approx -0.33$ is approached.  Around this transition the ratio is characterized by intermittent bursts of activity but with no tendency for the stock to be over- or under-valued.  Beyond the transition $r_p<r_2$ fluctuations dominate, but again with no evidence of bubbles or crashes.
 
\subsection{Summary}

In this section we found that CSEM exhibits clear evidence of crashes (but not speculative bubbles) when the control parameter $\sigma_\epsilon$ is set below the critical point.  DSEM also appeared to exhibit some weaker evidence of crashes (and bubbles) near its critical point but with larger fluctuations which prevented the over- and under-valuation of the stock for extended periods.

A much richer analysis of the phenomenon of bubbles and crashes in these models is possible but not worth the effort because it does not relate to empirical market data.  As mentioned above, it is extremely difficult to establish the existence of endogenous price bubbles and crashes in real markets because of the coupling with their environments.  Hence, further research in this area is largely pointless.  The above presentation was included because \edit{why?  helps understanding...was done in another paper \cite{arthur97}}


